Multi-antenna Coded Caching at Finite-SNR: Breaking Down the Gain Structure

Multi-antenna coded caching (CC) techniques are considered viable options for achieving higher data rates in future networks, especially for the prominent use case of multimedia-driven applications. However, despite their information-theoretic analyses, which are thoroughly studied in the literature, the research on the finite-SNR performance of multi-antenna CC techniques is not yet mature. In this paper, we try bridging this gap by breaking down, categorizing, and studying the effect of six crucial parameters affecting the finite-SNR performance of multi-antenna CC schemes. We also investigate the interaction of different parameters and clarify how they could affect the implementation complexity in terms of the necessary computation and subpacketization. Theoretical discussions are followed and verified by numerical analysis.

==> Data/CCMAC.tex <==
SNR	B10OPT	B5OPT	B2OPT	B1OPT	B10toB1OPT	B2toB1OPT	B5toB1OPT
0	3.019496031	3.237992628	3.050747707	2.928696004	3 	4 	11 
5	6.006190989	6.203754341	5.843921052	5.537773058	8 	6 	12 
10	10.05986468	10.15248871	9.617257408	9.103326084	11 	6 	12 
15	15.12031657	15.05797721	14.20208891	13.39369048	13 	6 	12 
20	21.17906799	20.85934331	19.47841259	18.23805437	16 	7 	14 
25	27.93463344	27.3101688	25.33555066	23.39801623	19 	8 	17 
30	35.03084845	34.15059121	31.62450906	28.8261219	22 	10 	18 


==> Data/CCMC.tex <==
SNR	P15OPT	P12OPT	P6OPT	P3OPT	P15toP3OPT	P12toP3OPT	P6toPeOPT
0	3.019496031	2.942123949	2.24876639	2.042137213	48 	44 	10 
5	6.006190989	5.682989345	4.483561279	4.064630863	48 	40 	10 
10	10.05986468	9.36986002	7.625063013	6.907223017	46 	36 	10 
15	15.12031657	14.05027524	11.79554043	10.66633933	42 	32 	11 
20	21.17906799	19.84333005	17.17364819	15.52134839	36 	28 	11 
25	27.93463344	26.57432536	23.62563627	21.43007544	30 	24 	10 
30	35.03084845	33.78025068	30.73168825	28.10399695	25 	20 	9 


==> Data/CCMUX.tex <==
SNR	t2OPT	t1OPT	t0OPT	t2tot0OPT	t1tot0OPT	t2tot0TH	t1tot0TH
0	3.019496031	2.545210477	1.722927977	75 	48 	50 	25 
5	6.006190989	4.816306824	3.158179176	90 	53 	50 	25 
10	10.05986468	7.888027322	5.013348108	101 	57 	50 	25 
15	15.12031657	11.82856724	7.360721638	105 	61 	50 	25 
20	21.17906799	16.6813452	10.32663768	105 	62 	50 	25 
25	27.93463344	22.24682991	13.92519769	101 	60 	50 	25 
30	35.03084845	28.16252698	18.02488853	94 	56 	50 	25 


==> Data/SBF.tex <==
SNR	A4OPT	A3OPT	A2OPT	A1OPT	A4toA1OPT	A3toA1OPT	A2toA1OPT	A4toA1TH	A3toA1TH	A2toA1TH
0	3.019496031	3.255389193	3.19462742	3.03884808	-1 	7 	5 	100 	67 	33 
5	6.006190989	6.344362273	6.195238781	5.633862543	7 	13 	10 	100 	67 	33 
10	10.05986468	10.54495756	10.12109494	8.766504708	15 	20 	15 	100 	67 	33 
15	15.12031657	15.68325763	14.54256121	12.12092439	25 	29 	20 	100 	67 	33 
20	21.17906799	21.33266891	19.13520889	15.54965486	36 	37 	23 	100 	67 	33 
25	27.93463344	27.14877531	23.76366594	19.00050556	47 	43 	25 	100 	67 	33 
30	35.03084845	32.9969125	28.39100504	22.45708665	56 	47 	26 	100 	67 	33 
35

==> Data/SMUX.tex <==
SNR	L4OPT	L3OPT	L2OPT	L1OPT	L4toL1OPT	L3toL1OPT	L2toL1OPT	L4toL1TH	L3toL1TH	L2toL1TH	L4toL3OPT	L4toL3TH	L4toL2OPT	L4toL2TH
0	3.019496031	2.49186387	1.423904776	0.597396735	405 	317 	138 	100 	67 	33 	21 	20 	112 	50 
5	6.006190989	5.008934723	3.162012335	1.512479737	297 	231 	109 	100 	67 	33 	20 	20 	90 	50 
10	10.05986468	8.497909094	5.709079172	3.223654597	212 	164 	77 	100 	67 	33 	18 	20 	76 	50 
15	15.12031657	12.96424947	8.899232124	5.738082738	164 	126 	55 	100 	67 	33 	17 	20 	70 	50 
20	21.17906799	18.26457795	12.76218425	8.807504004	140 	107 	45 	100 	67 	33 	16 	20 	66 	50 
25	27.93463344	24.06475332	17.17230996	12.16160646	130 	98 	41 	100 	67 	33 	16 	20 	63 	50 
30	35.03084845	30.04428564	21.91653976	15.63077287	124 	92 	40 	100 	67 	33 	17 	20 	60 	50 
35

==> Data/STYPE.tex <==
SNR	L4A4OPT	L4A4ZF	L4A2OPT	L4A2ZF	L4A4OPTtoZF	L4A2OPTtoZF
0	3.019496031	0.442695864	3.19462742	1.76642666	582 	81 
5	6.006190989	1.342893157	6.195238781	4.218965827	347 	47 
10	10.05986468	3.768993242	10.12109494	8.022700117	167 	26 
15	15.12031657	8.9253664	14.54256121	12.54641351	69 	16 
20	21.17906799	16.63372103	19.13520889	17.25074781	27 	11 
25	27.93463344	25.62381906	23.76366594	21.94334747	9 	8 
30	35.03084845	34.2407576	28.39100504	26.6036158	2 	7 


==> OldParameterExplanation.tex <==


In this extended summary, we briefly introduce the parameters listed in Figure~\ref{fig:gain_breakdown} and provide preliminary simulation results for each parameter. For the network setup, it is assumed that a single server with $L$ transmit antennas communicates with $K$ single-stream users, resulting in a multi-input single-output (MISO) scenario. The users request data from a library of $N$ files each with $F$ bits in size, and each user has a cache memory of size $MF$ bits. 

System operation consists of two phases, content placement and delivery. In the placement phase, users' cache memories are filled up with appropriate data. Then, in the delivery phase, after the users reveal their requested files, the server creates multiple transmission vectors and transmits them to the users in consecutive time slots. The aim is to design placement and delivery phases (together known as the CC scheme) such that after the transmissions, every user can decode its requested data and the total delivery time is minimized. We consider CC schemes with uncoded cache placement and single-shot data delivery, for which the CC scheme in~\cite{shariatpanahi2016multi,shariatpanahi2018physical} is known to be DoF-optimal~\cite{lampiris2018resolving}. Subsequently, unless otherwise mentioned, we use the same CC scheme and optimized beamformers for the simulations. The comparison metric is the symmetric rate, defined as the total data transferred over the channel divided by the total delivery time. Finally, the CC gain $t$ is defined as the total cache ratio, i.e., $t = K\frac{M}{N}$.
%, and the spatial multiplexing parameter is denoted by $1 \le \alpha \le L$.

%In the following, we provide a short descriptive explanation and simulation results for each of the parameters listed in Figure~\ref{fig:gain_breakdown}. We have used $K$ to denote the number of users and $L$ to represent the maximum values of spatial multiplexing gain at the transmitter (i.e., the rank of the channel matrix). Also, $t$ and $\alpha$ show the CC gain and the selected spatial multiplexing value, respectively. More detailed explanations are left for the extended version of the paper.

\noindent\textbf{Spatial multiplexing}, denoted by $\alpha$,
indicates at how many users the interference from each term can be nulled out (or suppressed) by beamforming vectors, and hence, directly affects the DoF. Even though $\alpha$ can be selected freely from the set $\{1,2,...,L\}$, for a fair analysis here we assume $\alpha = L$ as choosing $\alpha < L$ would also affect the beamformer directivity. Simulation results for a small network of $K=6$ users are provided in Figure~\ref{fig:smux_plot} and Table~\ref{tab:smux_bar}.


%As will be discussed, choosing $\alpha < L$ affects not only the spatial multiplexing but also the beamformer directivity, and hence, for a fair analysis we assume $\alpha=L$ while simulating its effect.
%Using $\alpha$ to denote the spatial multiplexing value, from communication theory we know that $1 \le \alpha \le L$. 
%Simulation results for the effect of $\alpha$ parameter for a small network of $K=6$ users with $t=2$ is provided in Figure~\ref{fig:smux_plot} and Table~\ref{tab:smux_bar}. For a fair analysis, optimized beamformers are deployed and it is assumed that $\alpha = L$ (as will be discussed, with $\alpha < L$, the beamformer directivity would be affected).

\noindent\textbf{Beamformer directivity}
indicates how well the beams are directed towards target users. As discussed in~\cite{tolli2017multi}, if $\alpha < L$, even though the inter-user interference is nulled out (or suppressed) at fewer users, the finite-SNR performance is improved as the beams would be better directed to the target users. This effect is shown in Figure~\ref{fig:sbf_plot} and Table~\ref{tab:sbf_bar}.

\noindent\textbf{Beamformer structure}
indicates whether or not the inter-user interference is nulled out completely by beamforming vectors. From~\cite{tolli2017multi}, we know that optimized beamformers provide much better performance at the finite-SNR regime compared with ZF, but the gap between the two is narrowed as the SNR is increased. This is illustrated in Figure~\ref{fig:stype_plot} and Table~\ref{tab:stype_bar}.

\noindent\textbf{CC-aided multiplexing}, is the same parameter as the CC gain $t$, and
indicates at how many users the interference from each term can be removed using their cached contents. 
%It is in fact the same parameter as the CC gain $t$. 
Similar to $\alpha$, $t$ also directly affects the DoF.
%We expect the performance to increase as $t$ is increased, and the improvement to be non-dependent on the SNR as no beamforming is involved. 
Simulation results for this parameter are provided in Figure~\ref{fig:ccmux_plot} and Table~\ref{tab:tmux_bar}.
%, for a network of $K=6$ users with $\alpha = L = 4$ where optimized beamformers are applied.

\noindent\textbf{CC-aided multicasting}
indicates how many users receive each codeword during the delivery phase. Pure signal- and bit-level CC schemes have the least and the most CC-aided multicasting, respectively~\cite{salehi2019subpacketization}. It does not affect the DoF but the performance and the beamformer design complexity~\cite{salehi2021low,mahmoodi2021low}. Simulation results can be found in Figure~\ref{fig:ccmc_plot} and Table~\ref{tab:ccmc_bar}, where $P$ denotes the subpacketization and larger $P$ allows more CC-aided multicasting~\cite{salehi2019subpacketization}.

%It also indicates to much extent the cache-aided interference cancellation is done in the signal domain. For CC schemes with the full signal-level approach such as the ones in~\cite{lampiris2018adding,salehi2021low}, there is no multicasting and all the interference is cancelled in the signal domain. However, there exist schemes such as ... where part of the interference is cancelled at the signal domain. As studied in~\cite{salehi2019subpacketization}, this parameter is affected by the subpacketization. So, in simulation results, we have used ...

\noindent\textbf{Superposition (MAC)}
indicates how many data terms should be simultaneously decoded by every user after each transmission slot. 
It affects both the finite-SNR performance and the beamformer design complexity~\cite{tolli2017multi,mahmoodi2021low}. Simulation results for the superposition parameter, denoted by $\beta$ here, are provided in Figure~\ref{fig:ccmac_plot} and Table~\ref{tab:ccmux_bar}.


%The original bit-level CC scheme in~\cite{shariatpanahi2016multi} required each receiver to decode ... terms after each transmission, necessitating a successive interference cancellation (SIC) receiver. However, SIC receivers are difficult to implement in practice. Moreover, as studied in~\cite{mahmoodi2021low}, if the CC scheme requires no SIC receiver, designing optmized beamformers could become much simpler even with multicasting. As discussed in~\cite{tolli2017multi}, we expect the MAC size to have little effect on the performance. This is verified in ... where the simulations are done for ...

%\textbf{Notations.}

%\textbf{Paper Structure.} In Section~\ref{section:sysmodel}, we review the system model and describe the considered beamforming strategies. Sections~\ref{section:misogains} and~\ref{section:ccgains} are devoted to explaining various gains and design decisions for MISO connectivity and CC part, respectively. The discussions in these two sections include clarifying simulation results. Finally, in Section~\ref{section:conclusion} we conclude the paper.

Network setup goes here
In all the simulations, we calculate both the rate and the simulation time.

\subsection{Coded caching scheme}

Every transmission vector delivers useful data to $t+\alpha$ users, simultaneously. Let us denote the transmission vector with target users $\CS \subseteq \CK$ as $\Bx_{\CS}$, where $|\CS| = t+\alpha$.
With every transmission vector $\Bx_{\CS}$, we transmit multiple codewords $X_{\CT}$, where $\CT \subseteq \CS$ and the codeword $X_{\CT}$ delivers useful data to every user $k \in \CT$. Depending on the scheme, number of users in each set $\CT$ can be different, but in general, $|\CT| \in [t+1]$.
\textbf{For respective section: the value of $\CT$ determines the cache-aided multicasting parameter and the number of $\CT$ sets including a specific users $k \in \CS$ determines the MAC parameter.} Every codeword $X_{\CT}$ is precoded using a beamforming vector $\Bw_{\CR(\CT)}$ that nulls-out (or suppresses) the interference of $X_{\CT}$ at every user in $\CR(\CT)$. So, in summary, the transmission vector $\Bx_{\CS}$ is built as
\begin{equation}
    \Bx_{\CS} = \sum_{\CT \in \Bar{\CT}(\CS)} X_{\CT} \Bw_{\CR(\CT)}.
\end{equation}
Then, at the receiver of user $k \in \CS$, we receive
\begin{equation}
    y_{\CS} (k) = \sum_{\CT \in \Bar{\CT}(\CS)} X_{\CT} {\Bh_{\CS}(k)}^H \Bw_{\CR(\CT)} + z_{\CS} (k),
\end{equation}
where $\Bh_{\CS}(k) \in \mathbb{C}^{L \times 1}$ is the channel vector and $z_{\CS} (k)$ represents the AWGN during the transmission of $\Bx_{\CS}$. For notational simplicity, we use $\Bh_k$ and $z_k$ to represent them afterwards. The user $k$ then has to decode every codeword $X_{\CT}$ where $\CT \ni k$ from $y_{\CS} (k)$, using appropriate techniques.

Let us denote the time required for every user $k$ in $\CS$ to decode $y_{\CS}(k)$ as $T_{\CS}$. Then, the total delivery time will be $T = \sum_{\CS} T_{\CS}$, and the symmetric channel rate, which is the parameter selected here for performance comparison, can be defined as
\begin{equation}
    R = \frac{K(1-t)}{T}.
\end{equation}
It should be noted that, in the literature, the total symmetric rate (which includes the effect of the local caching gain), is defined as $R_s = K/T$. Here, we use the symmetric channel rate in ... as we want to compare the effect of different parameters on how well we use the communication channel. Of course, the two rates can be converted into each other using a simple multiplication.

%The baseline network is with $K=6$ users, coded caching gain $t=3$, transmitter-side antenna count of $L=3$, and the spatial multiplexing gain of $\alpha = L$.

%It should be explained that we are considering the \textit{channel rate} and how it can be converted to the \textit{total symmetric rate}.

\subsection{Beamforming}
Various beamforming strategies for CC schemes are described in~\cite{tolli2017multi}. The discussion in~\cite{tolli2017multi} includes three different beamforming strategies; optimized, zero-force with power loading, and zero-force with equal power allocation. In this paper, we only consider the first two strategies as zero-force with equal power allocation provides poor performance at the entire SNR regime. Consequently, we use the abbreviated term ZF to refer to zero-force beamforming with power loading. 

\noindent\textbf{ZF Beamforming.}

\noindent\textbf{Optimized Beamforming.}

\subsection{The example network}
We consider a network of $K=6$ single-antenna, cache-enabled users. Either explicitly mentioned, we assume each user can cache a portion $\gamma=1/3$ of the entire library (i.e., $t=2$) and the transmitter has $L=4$ adequately-separated antennas. Clearly, with $L$ antennas at the transmitter, the spatial multiplexing parameter $\alpha$ can be any value in $[L]$. Finally, except otherwise noted, we assume optimized beamformers are used to suppress part of the interference at unwanted users.

==> wrapup.tex <==
For MISO-native parameters:
\begin{itemize}
    \item Having larger antenna arrays is always good as it adds a whole new resource to the system.
    \item For a fixed antenna array size, at the finite-SNR regime it is better to trade the spatial multiplexing gain with the beamformer directivity. Fortunately, this does not impose any structural changes to the underlying caching scheme, i.e., we do not need to design a new CC scheme. Moreover, it only affects the second-layer subpacketization (before the transmission), and hence, this parameter can be selected instantly and over the air. \textbf{This property should be kept in mind as we design new CC schemes.}
    \item As expected, optimized beamformers always outperform zero-forcing. However, the gap between the two strategies narrows down heavily at high-SNR. The gap can also be reduced at the finite-SNR regime by reducing the spatial MUX gain. So, reducing the spatial multiplexing gain at the finite-SNR regime has also another benefit: we can use less-complex ZF beamformers if complexity is a big issue.
    \item Designing less-complex optimized beamformer designs well-tailored for CC schemes is of much interest. One interesting work is done by Nariman in~\cite{mahmoodi2021low}. However, it only applies when the CC MAC size is one.
\end{itemize}

For CC-native parameters:
\begin{itemize}
    \item Similar to the antenna count, having more memory is always good as it adds a whole new resource to the system. There is one important difference, though: the gain from having more memory is less-dependent on the SNR and can be achieved regardless of the SNR value (which makes sense, as memory-aided interference cancellation has nothing to do with the SNR value).
    \item The CC multiplexing gain also plays an important role (up to 50\%) in the achievable performance. However, this is a tricky parameter to play with: on the one hand, we have pure signal-level CC schemes that provide lots of benefits such as handling dynamicity, reduced subpacketization, easy extension to MIMO setups, etc. and on the other hand are pure bit-level schemes that provide the highest multicasting gain and hence the highest possible performance. It is a big question whether this trade-off could be tuned more gently; i.e. whether we could have some benefits of the signal-level schemes while keeping at least part of the multicasting gain. For example, the easy beamformer design is shown to be doable for some bit-level schemes (Nariman), and reduced subpacketization is also shown to be possible somehow (Soheil and Itsik). A more thorough study is highly encouraged.
    \item Increasing the MAC size provides a very small benefit but adds much to the complexity. Specifically, it requires much more complex receivers. If removing the MAC makes bit-level schemes more flexible, e.g., by allowing simpler beamformer designs for them, we should aim for that.
\end{itemize}
